An optimized Space-Time Multigrid algorithm for parabolic PDEs

We investigate three directions to further improve the highly efficient Space-Time Multigrid algorithm with block-Jacobi smoother introduced in [GanNeu16]. First, we derive an analytical expression for the optimal smoothing parameter in the case of a full space-time coarsening strategy; second, we propose a new and efficient direct coarsening strategy which simplifies the code by preventing changes of coarsening regimes; and third, we also optimize the entire two cycle to investigate if further efficiency gains are possible. Especially, we show that our new coarsening strategy leads to a significant efficiency gain when the ratio $\tau/h^2$ is small, where $\tau$ and $h$ represent the time and space steps. Our analysis is performed for the heat equation in one spatial dimension, using centered finite differences in space and Backward Euler in time, but could be generalized to other situations. We also present numerical experiments that confirm our theoretical findings.

==> old/old.tex <==
\section{Introduction}
\label{intro}

% \begin{itemize}
%     \item Make sure to place our work in the context of Lars' previous cascadic MG work \cite{Haber_2017}
%     \item Justify the paper by arguing that we
%     \begin{itemize}
%         \item Need to know how to intelligently initialize a truly deep network, and demonstrate this, in order for layer-parallel to make any sense.  (In the future, we can look at truly multilevel optimization ideas)
%         \item This is slightly different from Lars' work in that we put cascadic MG in the context of an iterative layer-parallel solver.  We have found that Braid doesn't converge well after interpolation from a coarse network to a fine one.  And, we have to do extra Braid iterations for a few optimization steps.  We've also found that piecewise constant interpolation seems to be fine.  These are admittedly small things, though. 
%         \item  Another small novelty, is that we investigate cascadic multigrid as a "regularizing" force.  That is, our parameter searches seem to become less sensitive when using cascadic multigrid.
%     \end{itemize}
% \end{itemize}

We consider learning problems that are based on the continuous neural network formulation as in \cite{Haber_2017,ChRuBeDu2018}, and note that there has been considerable interest in related ODE- and PDE-inspired formulations as of late \cite{weinan2017proposal,chang2018reversible,chaudhari2018deep,lu2017beyond,ruthotto2018deep}. 
% \textcolor{red}{Any more references?} I'm cool 
In this setting, the neural network is cast as a time-dependent ordinary differential equation (ODE) which describes the flow of data elements $y_k \in \R^{n_f}, k=1,\dots,s$ (the \textit{feature} vectors) through the neural network as
\begin{align}
  \partial_t u_k(t) &= F(u_k(t), \theta(t)) \quad \forall t \in (0,T) \label{network_flow}\\
  u_k(0) &= L_{in}\response{(\theta(0))} y_k \label{network_init}.
\end{align}
Here, $u_k(t)\in R^w$ describes the state of a neural network of width $w$, and $\theta(t)\in\R^p$ represents the network parameters \response{that are to be learned during training}. $L_{in}$ maps the input feature vectors $y_k$ to the network dimension; the right-hand-side $F$ then determines the flow of the data element through the network. $F$ typically consists of an affine transformation that is parameterized by $\theta(t)$, and a nonlinear transformation that is applied element-wise using an {activation} function, i.e. 
\begin{align}
  F(u_k(t),\theta(t)) = \sigma(W(\theta(t)) u_k(t) + b(\theta(t))),
\end{align}
where $W(\theta(t))$ is a linear transformation, such as a convolution, applied to the state $u_k(t)$, \response{and} $b(\theta(t))$ is a bias added to the state. \response{$W$ and $b$ are parameterized by the network parameters $\theta(t)$, for example $\theta(t)$ can define entries for a dense weights matrix $W$ and a dense bias vector $b$}. \response{The function} $\sigma\colon \R \to \R$ denotes the nonlinear activation function \response{that is} applied component-wise, such as the ReLU activation $\sigma(x) = \max(x,0)$. \response{Similarly, $L_{in}(\theta(0))$ is an input layer where again the nonlinear activation function is applied to an affine transformation. The bias and weight matrix are defined by $\theta(0)$, and the weight matrix maps the input data to the size of the neural network and is thus not square.}

In contrast to traditional neural networks that transform the network state at prescribed layers, the continuous formulation prescribes the rate of change of the network state using an ODE parameterized by $\theta(t)$. This control function $\theta(t)$ is to be learned during training by solving a constrained optimization problem. For example, in supervised learning, the optimization problem aims to match the network output $u_k(T)$ to a desired output $c_k \in \R^{n_c}$ that is given from the training data set:
\begin{align} \label{eq:training}
  \min_{\theta} \, &\frac 1 s \sum_{k=1}^s \ell(  u_k(T), c_k) + \response{\gamma}\int_0^T R(\theta(t)) \, \mathrm{d} t \\
  \text{s.t. equations } &\eqref{network_flow}-\eqref{network_init} \mbox{ are satisfied } \forall \, k=1,\dots, s.
\end{align}
Here, $\ell$ denotes a loss function that measures the distance of the network output at final time $T$ to the desired output, and $R$ denotes a regularization term \response{with parameter $\gamma > 0$}, such as a Tikhonov regularization on $\theta(t)$ and/or its time derivative, that stabilizes the optimization problem numerically.
Training is generally considered successful, if the network parameters $\theta(t)$ generalize well to new, previously unseen data,
which is represented as a validation data set. 


To solve the neural network flow numerically, classical time-integration schemes are applied that discretize the ODE in equation \eqref{network_flow} on a given time-grid $0=t^1<\dots< t^N=T$, and solve the resulting equations one after another for each time step $t^i$. In this scenario, each time-step is associated with one layer of a classical artificial neural network, leading to the traditional network propagation with $u^n_k \approx u_k(t^n)$ \response{being the network state at layer $n$, and $\theta^n\approx \theta(t^n)$ the network parameters (weights and biases) at layer $n$}. In fact, it has been observed that many state-of-the-art artificial neural networks can be interpreted as discrete time-integration schemes of the parametrized ODE in equation \eqref{network_flow} (see e.g. \cite{LuZhLiDo2017}). For example, an explicit Euler scheme to discretize \eqref{network_flow} gives
\begin{align}
  u^{n+1}_k = u^n_k + hF(u_k^n, \theta^n), \label{eq:resnet}
\end{align}
which resembles the classical ResNet~\cite{HeZaReSu2016} with an additional time-step size $h>0$.  We note that $h=1$ in the classical ResNet.

The continuous network formulation opens the door for
leveraging various optimization schemes and optimal control theory that has been developed for ODE and PDE constraints \cite{Li1971,Tr2010,BiGhHeBl2003}.
In particular, stability analysis of explicit time-integration schemes suggests favoring many-layer networks utilizing a small step size $h$ in order to ensure a numerically stable network propagation. Networks based on numerical time-integration schemes can therefore easily involve hundreds or thousands of discrete layers (time-steps) \cite{GuRuScCyGa2018,ChRuBeDu2018,Haber_2017}. 

However, training very deep networks comes with both numerical and computational challenges. 
\response{Traditional parallel algorithms in machine learning, recently reviewed in~\cite{ben2019demystifying}, can be used to accelerate training for increasing the number of samples (e.g. batch size), or growing the width of the network. However, as the strong scaling limit is reached for these forms of parallelism the serial nature of time evolution creates a barrier for parallel scalability with increased network depth.}
If network states are propagated through the network in a serial manner, as is done with classical training methods, an increase in the number of layers (i.e. more time steps, and smaller steps sizes) results in an equally larger time-to-solution. In order to address this serial bottleneck, a layer-parallel multigrid scheme has been developed in \cite{GuRuScCyGa2018} to replace the serial forward and backward network propagation. In this scheme, the network layers are distributed onto multiple compute units, and an iterative multigrid method is applied to solve the network propagation equations inexactly in parallel, across the layers.  This iterative scheme converges to the same solution as serial network propagation.  The result is that runtimes remain nearly constant when the numbers of layers and compute resources are increased commensurately (weak scaling), and that runtimes can be significantly reduced for a fixed number of layers and increasing compute resources (strong scaling). The layer-parallel multigrid method will be summarized in Section \ref{sec:MGRIT}.

In addition, many-layer networks increase the complexity of the underlying optimization problem. In particular, considering more and more layers and hence more and more network parameters creates highly non-convex optimization landscapes which require proper initialization in order to be trained effectively. A number of schemes have been developed for initializing plain and residual neural networks. Commonly implemented techniques include Glorot~\cite{glorot10} and He~\cite{he2015delving}; however, this is still an active area of research, with new methods being proposed (e.g.~\cite{hanin2018start,humbird2018deep,boxinit2019}). 

In this paper, we investigate a multilevel network initialization strategy that successively increases the number of network layers during layer-parallel multigrid training. The first use of such a multilevel (or ``cascadic") initialization strategy for an ODE network was done in the context of layer-serial training in \cite{Haber_2017}.  Here, a sequence of increasingly deeper network training problems are solved, and each new deeper network is initialized with the interpolated learned parameters from the previous coarser network. We refer to this process as a ``nested iteration", because of this terminology's long history. Nested iteration broadly
describes a process (originally for numerical PDEs/ODEs) that starts by finding the solution for a relatively coarse problem representation, where the solution
cost is relatively cheap.  This coarse solution is then used as an inexpensive initial guess for the same problem, 
but at a finer resolution. Nested iteration was first discussed in a multigrid context at least in 1981
\cite{hackbusch1981convergence}, 
and the concept of nested iterations for solving numerical PDEs goes back at least to 
1972 \cite{kronsjo1972design,Kr1975}.  Nested iteration is often called ``full multigrid" in the
multigrid context, and famously provides optimal $O(n)$ solutions to some elliptic problems with $n$ unknowns 
\cite{BrHeMc2000,TrOo2001}. Nested iteration, especially when only regions with large error are marked for refinement, 
can lead to remarkably efficient solvers \cite{AdMaMcNoRuTa2011,DeMa2008}.  We will take advantage of this
inherent efficiency to cheaply find good initializations for ODE networks, by successively refining
the time grid of the ODE network, adding more time-grid levels to the multigrid hierarchy.

% PDE-verse References for NI-refinement: Solve → Estimate → Mark → Refine
% [24] P. Morin, R. H. Nochetto, and K. G. Siebert, Data oscillation and convergence of adaptive
%   FEM, SIAM J. Numer. Anal., 38 (2000), pp. 466–488.
% [25] P. Morin, R. H. Nochetto, and K. G. Siebert, Convergence of adaptive finite element
%   methods, SIAM Rev., 44 (2002), pp. 631–658.

In this work, we \response{use} the nested iteration (or cascadic) initialization idea in the context of an iterative layer-parallel multigrid solver, which re-uses the coarser grid levels during multigrid cycling. We investigate two interpolation strategies (constant and linear) and their influence on the layer-parallel multigrid convergence and training performance. We further \response{perform a preliminary study on} the effect of multilevel initialization as a regularization force, with the desire that deep network training can become less sensitive towards hyperparameters and variation in network parameter initializations.  In other words, the goal is that with a better initial guess for the network parameters, the training process becomes more robust and less sensitive.

